Generalized Linear Bandits with Local Differential Privacy

Contextual bandit algorithms are useful in personalized online decision-making. However, many applications such as personalized medicine and online advertising require the utilization of individual-specific information for effective learning, while user's data should remain private from the server due to privacy concerns. This motivates the introduction of local differential privacy (LDP), a stringent notion in privacy, to contextual bandits. In this paper, we design LDP algorithms for stochastic generalized linear bandits to achieve the same regret bound as in non-privacy settings. Our main idea is to develop a stochastic gradient-based estimator and update mechanism to ensure LDP. We then exploit the flexibility of stochastic gradient descent (SGD), whose theoretical guarantee for bandit problems is rarely explored, in dealing with generalized linear bandits. We also develop an estimator and update mechanism based on Ordinary Least Square (OLS) for linear bandits. Finally, we conduct experiments with both simulation and real-world datasets to demonstrate the consistently superb performance of our algorithms under LDP constraints with reasonably small parameters $(\varepsilon, \delta)$ to ensure strong privacy protection.

==> real_single_epsilon_5.tex <==
\nextgroupplot[
axis line style={white!15!black},
legend cell align={left},
tick align=outside,
tick pos=left,
title={Real Data ($\varepsilon=5$)},
grid = both,
yshift=-1.8cm,
grid style={line width=.1pt, draw=gray!10},
x grid style={white!80!black},
xlabel={Time},
xmin=-2375, xmax=49875,
xtick style={color=white!15!black},
y grid style={white!80!black},
ymin=-500.76277869248, ymax=6500.0183525421,
ytick style={color=white!15!black},
scaled y ticks={real:1000}
]

% \path [draw=LDP-OLS, fill=LDP-OLS, opacity=0.2]
% (axis cs:0,0)
% --(axis cs:0,0)
% --(axis cs:2500,80.5402561202414)
% --(axis cs:5000,103.569936288801)
% --(axis cs:7500,122.041265176483)
% --(axis cs:10000,135.494081660244)
% --(axis cs:12500,147.084383379479)
% --(axis cs:15000,159.92397409463)
% --(axis cs:17500,171.476091055721)
% --(axis cs:20000,181.643798773715)
% --(axis cs:22500,189.917068203675)
% --(axis cs:25000,199.450299456051)
% --(axis cs:27500,209.764548353065)
% --(axis cs:30000,219.981141030299)
% --(axis cs:32500,228.142620922002)
% --(axis cs:35000,235.699169827619)
% --(axis cs:37500,243.093080757429)
% --(axis cs:40000,250.225886143819)
% --(axis cs:42500,258.186113019807)
% --(axis cs:45000,265.014960600693)
% --(axis cs:47500,271.944433626868)
% --(axis cs:47500,382.916928576643)
% --(axis cs:47500,382.916928576643)
% --(axis cs:45000,371.598101311918)
% --(axis cs:42500,359.387386369047)
% --(axis cs:40000,346.56667726509)
% --(axis cs:37500,334.675071019717)
% --(axis cs:35000,321.14005783172)
% --(axis cs:32500,309.284203022234)
% --(axis cs:30000,298.481764139323)
% --(axis cs:27500,284.36362148221)
% --(axis cs:25000,269.544249936371)
% --(axis cs:22500,255.200475750766)
% --(axis cs:20000,241.217186012305)
% --(axis cs:17500,225.818385188753)
% --(axis cs:15000,207.834377754615)
% --(axis cs:12500,188.403414343779)
% --(axis cs:10000,170.204586884345)
% --(axis cs:7500,148.834632818924)
% --(axis cs:5000,124.164724912468)
% --(axis cs:2500,94.3864545568449)
% --(axis cs:0,0)
% --cycle;

\path [draw=LDP-GLOC, fill=LDP-GLOC, opacity=0.2]
(axis cs:0,0.500012121044782)
--(axis cs:0,0.499982721121801)
--(axis cs:2500,1104.82019294992)
--(axis cs:5000,2183.3954179134)
--(axis cs:7500,2618.09653653261)
--(axis cs:10000,2892.75074904942)
--(axis cs:12500,3139.70137153073)
--(axis cs:15000,3367.93751583698)
--(axis cs:17500,3580.25560627756)
--(axis cs:20000,3786.54521654247)
--(axis cs:22500,3981.61093460595)
--(axis cs:25000,4165.68967025102)
--(axis cs:27500,4342.59607367437)
--(axis cs:30000,4520.51044779934)
--(axis cs:32500,4689.21513928369)
--(axis cs:35000,4862.73441214709)
--(axis cs:37500,5028.9540268485)
--(axis cs:40000,5190.33124320897)
--(axis cs:42500,5350.06294707062)
--(axis cs:45000,5512.26637882123)
--(axis cs:47500,5665.81596738092)
--(axis cs:47500,5720.44732216427)
--(axis cs:47500,5720.44732216427)
--(axis cs:45000,5563.65570872164)
--(axis cs:42500,5404.49008165192)
--(axis cs:40000,5245.16493740331)
--(axis cs:37500,5080.89556418122)
--(axis cs:35000,4909.59604722526)
--(axis cs:32500,4736.95651776591)
--(axis cs:30000,4566.14684304691)
--(axis cs:27500,4385.8042654755)
--(axis cs:25000,4205.45097634792)
--(axis cs:22500,4015.38204586959)
--(axis cs:20000,3815.21452434339)
--(axis cs:17500,3610.33053921177)
--(axis cs:15000,3394.62935112487)
--(axis cs:12500,3165.10080110314)
--(axis cs:10000,2916.24124097169)
--(axis cs:7500,2643.22037735219)
--(axis cs:5000,2191.54879700299)
--(axis cs:2500,1111.96235159122)
--(axis cs:0,0.500012121044782)
--cycle;

\path [draw=LDP-SGD, fill=LDP-SGD, opacity=0.2]
(axis cs:0,0.322472697396664)
--(axis cs:0,0.0775250822930576)
--(axis cs:2500,133.363975370636)
--(axis cs:5000,270.710472602456)
--(axis cs:7500,402.56727179948)
--(axis cs:10000,525.390400878726)
--(axis cs:12500,655.919049179677)
--(axis cs:15000,782.058489243121)
--(axis cs:17500,907.753957973526)
--(axis cs:20000,1036.33047467003)
--(axis cs:22500,1163.72056469712)
--(axis cs:25000,1286.57877602135)
--(axis cs:27500,1408.82480967236)
--(axis cs:30000,1530.23021863881)
--(axis cs:32500,1652.40907241995)
--(axis cs:35000,1777.53138298684)
--(axis cs:37500,1902.13819543025)
--(axis cs:40000,2024.91648826396)
--(axis cs:42500,2150.36561684227)
--(axis cs:45000,2283.64876248065)
--(axis cs:47500,2406.39606764682)
--(axis cs:47500,3131.48176646936)
--(axis cs:47500,3131.48176646936)
--(axis cs:45000,2976.37789319972)
--(axis cs:42500,2813.68755330085)
--(axis cs:40000,2655.3695106442)
--(axis cs:37500,2493.71667993335)
--(axis cs:35000,2329.58267104026)
--(axis cs:32500,2160.84707262877)
--(axis cs:30000,1998.26523540053)
--(axis cs:27500,1827.56642958695)
--(axis cs:25000,1667.9802934087)
--(axis cs:22500,1502.70922948559)
--(axis cs:20000,1340.34567991028)
--(axis cs:17500,1176.14843315825)
--(axis cs:15000,1011.34694912586)
--(axis cs:12500,837.112396820623)
--(axis cs:10000,671.830395509986)
--(axis cs:7500,510.962993573358)
--(axis cs:5000,346.195451268328)
--(axis cs:2500,174.167645443342)
--(axis cs:0,0.322472697396664)
--cycle;

% \addlegendentry{LDP-UCB}

\addplot [very thick, LDP-GLOC, dotted]
table[row sep=crcr]  {%
0 0.499997421083292\\
2500 1108.39127227057\\
5000 2187.47210745819\\
7500 2630.6584569424\\
10000 2904.49599501055\\
12500 3152.40108631693\\
15000 3381.28343348093\\
17500 3595.29307274466\\
20000 3800.87987044293\\
22500 3998.49649023777\\
25000 4185.57032329947\\
27500 4364.20016957493\\
30000 4543.32864542312\\
32500 4713.0858285248\\
35000 4886.16522968617\\
37500 5054.92479551486\\
40000 5217.74809030614\\
42500 5377.27651436127\\
45000 5537.96104377144\\
47500 5693.1316447726\\
};
% \addlegendentry{LDP-GLOC}

\addplot [very thick, LDP-SGD, mark = x]
table[row sep=crcr]  {%
0 0.199998889844861\\
2500 153.765810406989\\
5000 308.452961935392\\
7500 456.765132686419\\
10000 598.610398194356\\
12500 746.51572300015\\
15000 896.70271918449\\
17500 1041.95119556589\\
20000 1188.33807729015\\
22500 1333.21489709135\\
25000 1477.27953471502\\
27500 1618.19561962966\\
30000 1764.24772701967\\
32500 1906.62807252436\\
35000 2053.55702701355\\
37500 2197.9274376818\\
40000 2340.14299945408\\
42500 2482.02658507156\\
45000 2630.01332784019\\
47500 2768.93891705809\\
};
% \addlegendentry{LDP-SGD}

% \addplot [very thick, LDP-OLS, mark = |]
% table[row sep=crcr]  {%
% 0 0
% 2500 87.4633553385431\\
% 5000 113.867330600635\\
% 7500 135.437948997704\\
% 10000 152.849334272295\\
% 12500 167.743898861629\\
% 15000 183.879175924623\\
% 17500 198.647238122237\\
% 20000 211.43049239301\\
% 22500 222.55877197722\\
% 25000 234.497274696211\\
% 27500 247.064084917637\\
% 30000 259.231452584811\\
% 32500 268.713411972118\\
% 35000 278.419613829669\\
% 37500 288.884075888573\\
% 40000 298.396281704455\\
% 42500 308.786749694427\\
% 45000 318.306530956305\\
% 47500 327.430681101756\\
% };
